On the effect of time-dependent inhomogeneous magnetic fields in electron-positron pair production

Electron-positron pair production in space- and time-dependent electromagnetic fields is investigated. Especially, the influence of a time-dependent, inhomogeneous magnetic field on the particle momenta and the total particle yield is analyzed for the first time. The role of the Lorentz invariant $\mathbf{E}^2 - \mathbf{B}^2$, including its sign and local values, in the pair creation process is emphasized.

==> author_list.tex <==

\affiliation{Institut f\"ur Physik, Karl-Franzens-Universit\"at, A-8010 Graz, Austria}
\affiliation{Theoretisch-Physikalisches Institut, Abbe Center of Photonics, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany}

%
\author{Christian Kohlf\"urst} 
\email{christian.kohlfuerst@uni-jena.de}
\affiliation{Theoretisch-Physikalisches Institut, Abbe Center of Photonics,
Friedrich-Schiller-Universit\"at Jena, Max-Wien-Platz 1, D-07743 Jena, Germany \\ 
Helmholtz-Institut Jena, Fr\"obelstieg 3, D-07743 Jena, Germany}
\author{Reinhard Alkofer} 
\email{reinhard.alkofer@uni-graz.at}
\affiliation{Institut f\"ur Physik, Karl-Franzens-Universit\"at, A-8010 Graz, Austria}

%\noaffiliation
%
\vskip 0.25cm

